Causative Insights into Open Source Software Security using Large Language Code Embeddings and Semantic Vulnerability Graph

Open Source Software (OSS) security and resilience are worldwide phenomena hampering economic and technological innovation. OSS vulnerabilities can cause unauthorized access, data breaches, network disruptions, and privacy violations, rendering any benefits worthless. While recent deep-learning techniques have shown great promise in identifying and localizing vulnerabilities in source code, it is unclear how effective these research techniques are from a usability perspective due to a lack of proper methodological analysis. Usually, these methods offload a developer's task of classifying and localizing vulnerable code; still, a reasonable study to measure the actual effectiveness of these systems to the end user has yet to be conducted. To address the challenge of proper developer training from the prior methods, we propose a system to link vulnerabilities to their root cause, thereby intuitively educating the developers to code more securely. Furthermore, we provide a comprehensive usability study to test the effectiveness of our system in fixing vulnerabilities and its capability to assist developers in writing more secure code. We demonstrate the effectiveness of our system by showing its efficacy in helping developers fix source code with vulnerabilities. Our study shows a 24% improvement in code repair capabilities compared to previous methods. We also show that, when trained by our system, on average, approximately 9% of the developers naturally tend to write more secure code with fewer vulnerabilities.

==> sections/1_introduction.tex <==


The widespread dependency on OSS, ranging from IoT \cite{al2022idetect} operating platforms to essential software supply chains \cite{ladisa2023sok}, positions OSS as a very attractive target for cyber adversaries. Recent breaches, such as the compromise of SolarWind's Orion platform \cite{peisert2021perspectives} affected approximately 18,000 stakeholders, including major government bodies and critical infrastructure providers, shed light on the significant consequences of such cyber intrusions. These incidents highlight the vulnerabilities existing in widely-used software libraries \cite{log4j}, which can lead to extensive service disruptions \cite{synopsysrisc, log4j}. The interdisciplinary Open-Source Software Security Initiative (OS3I) was created in response to these challenges. OS3I includes agencies such as CISA, NSF, DARPA, and NIST intending to develop software security guidelines and robust security measures \cite{fedreg}. Building upon these security measures, it has become increasingly important to consider the impacts of technological innovations in the software development realm.



The software development landscape is becoming increasingly complex with the emergence of new technologies such as large language models, for example, GPT-4. While these technologies can streamline code development, they can also introduce significant security challenges \cite{khoury2023secure, sandoval2022security}, especially when the generated code goes to production without further verification. One of the most pressing challenges is the widespread accessibility of open-source code repositories or large language code generators. Although these resources can be invaluable for novice developers, facilitating faster progress and broader participation, they also present potential avenues for adversaries to inject vulnerabilities into software  \cite{democr1, democr2}. Studies in the literature indicate that nearly 40\% of open-source code resources, may fall short of proper security standards \cite{pearce2022asleep} for a software application. Moreover, the data used to train large language code models originates from publicly available insecure code repositories. This drawback highlights the crucial role of developer proficiency in code security to mitigate these risks. Yet, it is essential to recognize the challenges faced by developers, with some narratives framing them as potential ``weakest link in the chain" \cite{green2016developers} in software security.  Current research emphasizes the need for robust security support and developer training \cite{green2016developers, acar2016you}. Surveys conducted by Assal et al. \cite{assal2019think} and Hermann et al. \cite{weir2020needs} echo this sentiment, revealing gaps in developers’ understanding of security practices and a lack of access to security experts. Proactively addressing these issues becomes imperative to enhance the overall security posture of software development.


However, secure software development is complex and challenging, especially in the face of evolving technologies and cyber threats. In recent years, there has been a surge in automated vulnerability detection techniques \cite{zhou2019devign, li2018vuldeepecker, li2021vuldeelocator} in static source code, especially those based on transformer models \cite{nguyen2021regvd, islam2023unbiased}. Transformer methods can learn patterns in source code to identify potential vulnerabilities. A newer approach uses graph convolutional networks (GCN) \cite{guo2020graphcodebert}, which can help security analysts determine specific vulnerability types. Another promising area is automated vulnerability repair (AVR) \cite{pearce2023examining, joshi2023repair, chen2022neural} systems powered by generative models \cite{2020t5, wang2021codet5, touvron2023llama, zelikman2023self}, which can autonomously generate recommendations for fixing vulnerable code. Automated vulnerability detection tools are essential for fending off cyber threats. However, they face challenges such as the diversity or complex business logic of source code, the evolving nature of cyber threats, the lack of comprehensive datasets, and the need for human expertise. One key challenge is that current techniques, while good at classifying and locating vulnerabilities, do not provide developers with enough diagnostic information to fix them quickly and effectively.

% Need to connect with prev. paragraph

Recent user-focused research suggests that software developers often need various diagnostic information when addressing security challenges \cite{acar2016you, green2016developers}. While current vulnerability classification and localization play a critical role in discerning the specific location of code runtime failure, they cannot determine the true reason for the runtime failure, which is the \emph{root cause} of the vulnerability. This problem is further exacerbated within large-scale applications, potentially comprising millions of lines of code, where crash reproduction can be exceptionally challenging due to environmental discrepancies \cite{bellare1997forward, capobianco2019employing, han2020unicorn} of the system. Although capturing program stack traces or logs \cite{ji2017rain, kang2011dta} might provide insights such as vulnerability-causing inputs or code break locations, the derived results are often incomplete as they do not necessarily identify the root cause of the vulnerability. Consequently, these run-time analyses from stack traces are incredibly lengthy, needing more time (from developers) to sort them out, thus diminishing its usability as it requires too much back and forth between code writing and full deployment.




To clearly understand the limitations of previous systems and the needs of developers, we conducted a usability analysis through an extensive survey with participants majoring in Computer Science from an R1 Research University. Our analysis revealed that existing automated vulnerability detection techniques often fail to provide developers with a clear understanding of the root cause and their classification and localization of vulnerabilities. This hinders developers' ability to repair vulnerabilities and effectively write more secure code. To address these shortcomings, we introduce \emph{T5-GCN}, a novel approach for root cause diagnostics of software vulnerabilities. T5-GCN leverages the power of a large language model (LLM) and a graph convolutional network (GCN) to identify the root cause of vulnerabilities and classify and localize them with an added static description in the source code. Additionally, T5-GCN integrates an explainability-based approach to facilitate extracting relationships between vulnerable statements and the pivotal contributors to the vulnerability's root cause. We conducted another human-centric analysis to evaluate our approach's efficacy and practical implications. The results demonstrate that T5-GCN can effectively aid developers in rectifying vulnerabilities and enhancing their proficiency in crafting more secure code. Moreover, T5-GCN demonstrated robustness in discerning the root causes of N-day and zero-day vulnerabilities. Overall, T5-GCN presents an innovative approach for root cause analysis of software vulnerabilities. 

%It has the potential to significantly contribute to the field of software security by enabling developers to rectify vulnerabilities and craft more secure code. 


Thus, the main contributions of this paper are as follows:
\begin{itemize}

    \item  We present a foundational analysis conducted via a user survey to gauge the proficiency in secure coding among computer science graduates. Furthermore, we explore the limitations of existing code security vulnerability tools from the developers' perspective, particularly in aiding them in repairing vulnerabilities in their code. Our primary analysis emphasizes the necessity of understanding the root causes of vulnerabilities as a key element in empowering developers to address and resolve these security challenges successfully.
    %\item We present an introductory user survey-based analysis to determine the flaws of the current systems in assisting developers and analyze the shortcomings of the developers on code security knowledge. This primary analysis concludes that the root cause of the vulnerability is needed to help developers solve the vulnerability.

    \item We propose an LLM-based framework called T5-GCN, which employs explainability techniques to classify (by providing a CWE number and a short static description of the vulnerability category) and locate vulnerabilities along with the root cause. Furthermore, we performed an extensive evaluation with human subject participants to measure the effectiveness of our system compared to previous ones.

    \item We provide numerical analysis to show the quantitative results of our system. Furthermore, we also demonstrate the generalizability of our proposed approach by identifying N-day and 0-day vulnerabilities with their root cause in various open-source applications.


 
    
\end{itemize}

Our data and source code are publicly available \footnote{\url{https://anonymous.4open.science/r/Threat_Detection_Modeling-BB7B/README.md} }.
%\footnote{Test}   
    
%\color{red}

% General Challenge of Cyberattack on Code
\begin{comment}
    
In an era of escalating cyber threats, the Open Source Software (OSS) community stands at an unprecedented crossroads, charged with safeguarding the very foundation of countless software libraries, ranging from I/O operating platforms to essential software supply chains. Significantly, these libraries extend beyond mere supplementary tools; they form the core infrastructure for enterprises globally, emphasizing their pervasive adoption and indispensable value.
%The escalating frequency of severe cyberattacks on a global scale has disrupted the Open Source Software (OSS) community significantly, causing widespread downstream detrimental effects. 
However, security vulnerabilities in commonly used software libraries may lead to extensive service disruptions\cite{synopsysrisc}. In the aftermath of the Log4Shell incident \cite{log4j}, an interdisciplinary consortium, the Open-Source Software Security Initiative (OS3I), was formed to mobilize agencies such as the Cybersecurity Infrastructure Security Agency (CISA), National Science Foundation (NSF), Defense Advanced Research Projects Agency (DARPA), and National Institute of Standards and Technology (NIST) to delineate software security priorities and formulate cohesive policies collaboratively \cite{fedreg}. %Whether it is open-source or not, code security in a software ecosystem is a paramount concern that demands rigorous attention, concerted efforts, and innovative solutions for private entities and large enterprises.

%enabling more people to engage in 
The landscape grows more intricate with emerging technologies like ChatGPT, which despite enhancing developers' coding ability, introduces significant security challenges.
%While OSS and the recent advent of ChatGPT have accelerated the programming capabilities of developers, it has brought some security challenges 
\cite{khoury2023secure, sandoval2022security}. Open source code being highly accessible, novice developers are likely to use this code to complete the functionality of their coding task. Although this democratization of coding has increased the developers' productivity by enabling more people to engage in programming \cite{democr1, democr2}, open-source code available online or produced by large language models, often fails to meet software security standards, potentially containing vulnerabilities in around 40\% of cases. \cite{pearce2022asleep}.
More concerning is the training data of generative AI models, deeply rooted in the same insecure public repositories. 
%As a result, unless trained explicitly with security in mind, generative AI models (for automated code generation) gives rise to a vicious cycle of generating and disseminating more insecure code. Since the use of external code persists from novice to experienced developers, the possibility of spreading vulnerable code across various applications remains high.



Security issues can permeate within a application during different phases of its software development lifecycle. The ideal development lifecycle of a software application includes design, implementation, developer testing, code analysis, and code review phases \cite{assal2018security}. While the developer testing and code analysis phase contribute to functional testing of the code, security or vulnerability testing of code occurs primarily during the code review phase. \mj{I am not sure what is the point of the lines appearing before?} While security is sometimes seen as a burden in startup companies, in larger companies, it is considered a necessary evil to protect the company's products. Larger companies properly manage software development lifecycle, but small businesses or startups need to adequately implement better cyber security practices; otherwise, it leaves them susceptible to cyber-attacks \cite{chidukwani2022survey}. It is reported that about 60\% of small businesses that were victims of cyberattacks went out of business within six months \cite{galvin2021percent}. This report further demonstrates that small businesses have much to lose if cyber threats materialize, and it is in their best interest to have cyber defenses in place. Research highlights that 28\% of non-compliant victims will likely suffer another breach within two years after the initial attack \cite{vikingcloud} \mj{How is the last sentence related to everything before that? Appears out of place}.


% Issue with developers
While the democratization of code helps with faster progress, the cost of cybersecurity slows down their productivity in the long run.
Code security knowledge among developers plays a crucial role in ensuring the resilience of programs against various attacks. However, it is crucial to acknowledge developers' challenges as they are often seen as "the weakest link in the chain" regarding security \cite{green2016developers}. Developers are responsible for making final decisions on which code goes into production. Recent research highlights the need for comprehensive security support and training for software developers to effectively address these issues \cite{green2016developers, acar2016you}. One study by Assal et al. \cite{assal2019think} specifically examined the human factor in source code security. The survey highlighted the inadequate interaction between software developers and security practices. Similarly, Hermann et al. \cite{weir2020needs} conducted another survey revealing that less than a quarter of 335 successful mobile application developers had access to security experts. Therefore, addressing these issues is crucial to enhancing software development's overall security posture.




At the same time, recent user-focused research suggests that software developers need critical support when addressing security challenges \cite{acar2016you, green2016developers}. While current vulnerability classification and localization play a critical role in discerning the specific location of code failure, they cannot determine the root cause of the vulnerability. \mj{A sentence here describing what we intuitively mean by ``root cause" would help!} This problem is further exacerbated within large-scale applications, potentially comprising millions of lines of code, where crash reproduction can be exceptionally challenging due to environmental discrepancies \cite{bellare1997forward, capobianco2019employing, han2020unicorn} of the system. Although capturing program stack traces or logs \cite{ji2017rain, kang2011dta} might provide insights such as vulnerability-causing inputs or code break locations, the derived results are often incomplete as they do not necessarily identify the root cause of the vulnerability. Consequently, these run-time analyses from stack traces are incredibly lengthy. So they need time to sort them out, diminishing the usability of this method since it requires too much back and forth between code writing and full deployment.



%Our proposed system is the first to integrate an IoT operating systems repository scanner for function extraction using Joern \cite{joern} and a large language model VulCodeT5 to generate descriptions for the developers in repairing vulnerabilities. 
Therefore, in order to clearly understand what the previous systems are missing and what a developer needs, we initially do an extensive survey analysis. The analysis shows the drawbacks of current systems and reveals that a developer needs to understand the root cause of the vulnerability with a proper description of its CWE category. Thus, to find the root cause of the vulnerability, we introduce T5-GCN, a large language model combined with a Graph Convolutional Network (GCN), to find the root cause of the vulnerability along with its classification and localization. Our innovative approach incorporates an explainability-based method to extract the relationship between a vulnerable statement and the statement most contributing to the vulnerability's root cause. Afterward, we conduct a human evaluation to test the usability of our root cause analysis to repair vulnerabilities and how it intuitively increases the developer's knowledge in writing more secure code in the future. Furthermore, we test our system's generalizability by identifying the root cause of N-day and zero-day vulnerabilities. 

%\mj{Talk a bit more about the user study and the study's novelty. That is one of the most important aspect of the paper!}



%To address these challenges, we are the first to introduce VulCodeT5, a large language model for vulnerability localization and causative insights into the vulnerability. Our proposed VulCodeT5 provides GCN \cite{kipf2016semi} architecture powered by a CodeT5 embedding \cite{wang2021codet5} for vulnerability classification and localization, which harnesses the sequential/syntactical structure of tokens and the graphical structure of a programming language, respectively. Furthermore, we incorporate an explainability-based method to extract the relationship between a vulnerable statement and the statement most contributing to the vulnerability's root cause. The efficacy of our system is substantiated through an exhaustive case study \mj{why do you call it a ``case study"? are you evaluating just one use-case here?} analysis, focusing on evaluating 1) the model's classification performance and vulnerable line detection, 2) the effect of the outcome on the developers in writing secure code, and 3) demonstrating the application of our system by identifying the root cause analysis of vulnerability and its ability to identify and localize N-day and zero-day vulnerabilities in the wild. \mj{Talk a bit more about the user-study and the novelty of the study. That is one of the most important aspect of the paper!}


The contributions delineated in this paper are as follows:
\begin{itemize}

    \item We propose an introductory survey analysis to determine the flaws of the current systems and the drawbacks to the developers' security knowledge. Our primary analysis concludes that the root cause of the vulnerability is needed to help developers solve the vulnerability.

    \item In order to find the root cause of vulnerability, we proposed a T5-GCN(Temp. name) that can find the root cause of a vulnerability along with its classification and localization of the existing vulnerability. Furthermore, we do another extensive human evaluation to determine the effectiveness of our system compared to previous ones.

    \item We provide numerical analysis to show the quantitative results of our system. Furthermore, we also test the generalizability of our system in N-day and 0-day applications to identify the root cause of vulnerability in a program.
    
    %\item We introduce a system that performs function-level granularity analysis in source code to classify and localize vulnerabilities using a CodeT5-powered GCN architecture. This includes a novel token-based approach for finding vulnerable blocks of code.
    
    %\item We incorporate an explainability (used different terminology-- root cause/attribution/causal insight-- remove from the introduction) method within our system to identify the root cause of a vulnerability by elucidating the relationship between two statements: one engendering the vulnerability and the other instigating the code break.
    
    %\item We demonstrate a comprehensive use case of our system by demonstrating its effect on software developers. We provided an extensive survey analysis to demonstrate the usability of our system on its effect on developers and how it helps to write better and secure code.
    
    %detecting N-day and zero-day vulnerabilities prevalent in widely used IoT operating systems.
    
    
\end{itemize}
%\vspace{-11mm}

%The organization of the remainder of this paper is outlined as follows: In Section II, we dive deep into the motivation of this work. Then we delve into the relevant literature and previous studies in Section III. Section IV outlines our preliminary work on vulnerability exploitation, setting the groundwork for the subsequent sections. Our innovative methodology is thoroughly discussed in Section V. Section VI then provides an in-depth exposition of our experimental design and results, along with a comprehensive discussion of the findings. We further substantiate our findings with an ablation study, detailed in Section VII. We conclude our work, summarizing our contributions and discussing potential future directions in Section VIII.

%\vspace{-11mm}
\end{comment}


==> sections/7_threats_validity.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[b]
\centering
\caption{Ablation study on the Contrubution of each model}
%\vspace{0.3cm}
%\begin{tabular}{@{}cccccc@{}}
\begin{tabular}{p{0.04\textwidth}
                 p{0.08\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}}
\toprule
\textbf{Data} & \textbf{Model} &\textbf{IoU}  &\textbf{Acc.} & \textbf{F1} & \textbf{Pre.} & \textbf{Rec.} \\ \midrule



\multirow{3}{*}{D2A}           & GCN   & 0.52     & 0.59  & 0.58  &\textbf{0.70}  & 0.50        \\                          
                               & VulCodeT5   & 0.53      & 0.54    & 0.64 & 0.56          & 0.60\\
                               
                               & \textbf{VulCodeT5}   & \textbf{0.72}      & \textbf{0.62}    & \textbf{0.68} & 0.60          & \textbf{0.65} \\
\toprule
\multirow{3}{*}{BigVul} & GCN  & 0.39    & 0.58          & 0.57              & \textbf{0.70}              & 0.61              \\

    & VulCodeT5 & 0.42 & 0.60          & 0.57          & 0.58          & 0.60          \\
    & \textbf{VulCodeT5}   & \textbf{0.49}      & \textbf{0.65} &  \textbf{0.62} & 0.66 & \textbf{0.66} \\

                               
\bottomrule
\end{tabular}


\label{tab:crossval}
\end{table}








To analyze the individual contributions and assess the impact of different components in our IoT OS code vulnerability analysis system, we conducted an ablation study, systematically evaluating the effectiveness of various key factors and their influence on overall performance.

%We provide an ablation study to understand the effectiveness of each component of our ensemble model.

%\vspace{-2.0mm}



\subsection{Effectiveness of Combined Learning Ensemble Model}

To demonstrate the superiority of our ensemble model, we built and tested our models using VulCodeT5 (encoder) or GCN only for comparison. Our experimental results in Table \ref{tab:crossval} indicate that for vulnerability localization, the IoU value increases by at least 4\% compared to using GCN or VulCodeT5 (encoder) alone for both datasets. Additionally, we observe a 4\% increase in the F1 score for the vulnerability classification task for D2A dataset. Thus, our ablation study confirms that our ensemble model outperforms in both vulnerability classification and locating the vulnerable line.


\begin{figure*}[t]
    %\begin{framed}
        \centering
        
        \includegraphics[width=0.75\textwidth]{images/ablation_chart.pdf}
        
    %\end{framed}
    
    \caption{Multiclass classification of vulnerability by varying the contribution of each component of our ensemble model}
    \label{fig:chart_abl}
\end{figure*}

\subsection{Importance of Individual Embedding Generated by Our Ensemble Model}
The goal of an ensemble model is to combine several individual models to achieve superior performance. The ability to bring diverse data to fit into a model shows the diverse capabilities of an ensemble model. Therefore, we took the average embedding generated from VulCodeT5 (encoder), $F_R$, and GCN $F_{GCN}$ in our training and inferencing step.

However, our dataset has a good mix of different categories of vulnerabilities, some of which are more easily detectable by a GCN model and some using transformers. Therefore, to understand how each model contributes to our model's detection and localization capability, we multiply the embedding with varying constants $\kappa$ and $\lambda$ from Equation \ref{eqn:8}. We vary the value of $\kappa$ and $\lambda$ from 0 to 1, so their sum is always 1. When the value of $\kappa$ is lower/higher compared to $\lambda$, we see an increase/decrease in performance, indicating that one has more effect on the performance than the other. When any of the values of $\kappa$ or $\lambda$ is zero, it is equivalent to not using the model for classification and localization purposes.





From Table \ref{tab:abl_1}, we can see that the although we observe higher accuracy with 20:80 of VulCodeT5 (encoder) and GCN, we see a significant drop in F1 scores for this case in both D2A and BigVul datasets. We also observe that when the ratio goes close to 1, there is an improvement in the F1 scores, and when the ratio is 50:50, we achieve the highest F1 scores concluding the effectiveness of our ensemble model. We also see a similar trend for IoU scores, which peak when the ratio is 50:50.







\begin{comment}
    
    \begin{figure}[b]
    %\begin{framed}
        \centering
        
        \includegraphics[width=0.5\textwidth]{images/case_study_ablation.pdf}
        
    %\end{framed}
    
    \caption{An ablation study on the comparison of Attention score as an explainable technique with DeepLiftSHAP}
    \label{fig:cs_a}
\end{figure}

\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[b]
\centering
\caption{Ablation study on the contribution of each component of the ensemble model}
\begin{tabular}{@{}clllllll@{}}
\toprule
\multicolumn{1}{l}{\textbf{Dataset}} & \textbf{VulCodeT5} & \textbf{GCN}  & \textbf{IoU} & \textbf{Acc}  & \textbf{F1}   & \textbf{Pre.} & \textbf{Rec.} \\ \midrule
\multirow{5}{*}{D2A}        & 0.20   & 0.80 & 0.69 & \textbf{0.65} & 0.49 & 0.57 & \textbf{0.65} \\
                            & 0.40   & 0.60 & 0.68 & 0.61 & 0.54 & 0.58 & 0.60 \\
                            & 0.60   & 0.40 & 0.65 & 0.60 & 0.59 & 0.59 & 0.60 \\
                            & 0.80   & 0.20 & 0.67 & 0.59 & 0.46 & 0.53 & 0.59 \\ 
                            & 0.50   & 0.50 & \textbf{0.72} & 0.62 & \textbf{0.68} & \textbf{0.60} & 0.65 \\
                            \midrule
\multirow{4}{*}{BigVul}     & 0.20   & 0.80 & 0.46 & \textbf{0.71} & 0.59 & 0.55 & \textbf{0.71}    \\
                            & 0.40   & 0.60 & 0.46 & 0.66 & 0.62 & 0.61 & 0.66    \\
                            & 0.60   & 0.40 & 0.44 & 0.63 & 0.61 & 0.61 & 0.63    \\
                            & 0.80   & 0.20 & 0.45 & 0.62 & 0.60 & 0.61 & 0.62    \\
                            & 0.50   & 0.50 & \textbf{0.49} & 0.65 & \textbf{0.64} & \textbf{0.62} & 0.66    \\ \bottomrule
\end{tabular}
\label{tab:abl_1}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We further investigated the outcome of multiclass vulnerability detection and compared the F1 scores of the ensemble models when the model's different ratios were considered. Figure \ref{fig:chart_abl}, shows a distinction among the F1 scores of each class. For some CWE classes like CWE-119, CWE-20, CWE-125, and CWE-189, we see an upward trend in the F1 scores than the contribution of the GCN model is higher. This also explains that these vulnerabilities are memory-related and hence can be easily detectable by the GCN model. However, for the rest of the vulnerabilities, we see a downward trend when the contribution of VulCodeT5 (encoder) is lessened, concluding the effectiveness of VulCodeT5 (encoder) in classifying these vulnerabilities. This also explains higher accuracy, although lower F1 scores when we use the 20:80 ratio on the ensemble model in Table \ref{tab:abl_1}.





%\subsection{Ablation study on Root Cause analysis through explainability}

%To understand the effectiveness of our root cause of vulnerability analysis technique using DeepLiftShap, we use an inbuilt explainable property of the transformers called the attention values. The attention score evaluates the strength of a token's relationship with the other words in the sequence, providing a causal relationship between two tokens. We extract the values from all the attention heads into a single vector, thus getting equivalent scores for each line. However, attention values do not have a lower and upper limit than the DeepLiftShap scores. Therefore, after getting attention scores for all the lines, we convert them between the range of 0 to 1 and use these numbers with Algorithm \ref{alg:algorithm} to determine the root cause.

%Our analysis in Figure \ref{fig:cs_a} shows that, although in this example, we were able to determine localization for functions, it has some errors. According to Algorithm \ref{alg:algorithm}, line 1-4  is the root cause of vulnerability based on the attention scores. However, this is an incorrect prediction since line 1 is not a root cause of vulnerability. It is the declaration line of a function; hence, it can be neither a vulnerable line nor a line that is the root cause of a vulnerability. However, using DeepLiftSHAP, we get the correct lines (2-4) as the root cause of vulnerability.

%We provide a further ablation study in Appendix \ref{appendix}
















%In order to show that our ensemble model works better, we build a model using only RoBERTa or GCN. Our experimental results from Table \ref{tab:crossval} shows that for vulnerability localization, the IoU value has increased up to 5\% compared with GCN or RoBERTa. We also see an F1 score increase of 4\% for the vulnerability classification task. Hence our ablation study concludes that our ensemble model performs better in vulnerability classification and finding the vulnerable line.













==> sections/Arezou_Survey_Background_part.tex <==
\section{Background and Related Work}

During the post-deployment security testing of open-source applications, threat actors can exploit potential vulnerabilities, often arising from unintended backdoors left open by software developers.
Proactive security measures, including static code testing before deployment, are essential to ensure that code is resilient against various attacks, offering substantial savings in both time and costs. However, a significant gap exists due to inadequate interaction between software developers and security experts \cite{assal2019think}. Often viewed as the weakest link in the security chain, developers encounter challenges in creating secure code. This situation underscores the urgent need for comprehensive security support and training \cite{green2016developers, acar2016you}.
Current static application security analysis tools are instrumental but have limitations, which we discuss in section 2.4. They are often not generalized across different applications and lack actionable recommendations to assist developers in effectively addressing identified vulnerabilities.
In our exploration of the State-Of-The-Art (SOTA) techniques, it becomes apparent that there is a significant gap in the training of developers in code security. We evaluate the utility of current methods like VELVET \cite{ding2021velvet}, VulChecker \cite{mirskyvulchecker}, and LineVul \cite{fu2022linevul} in this context. These methods typically indicate the class and location of the vulnerability but fall short of offering actionable insights for remediation. In our study, we use these cutting-edge tools to identify threats.
To assess the practicality of the information provided by these SOTA techniques, we present developers with a vulnerable code snippet indicating the specific line and class of vulnerability, mirroring the output of VELVET, VulChecker, and LineVul. We then evaluate the developers’ ability to mitigate the identified vulnerabilities based on the provided information, aiming to glean insights into the efficacy of these tools in real-world applications and the enhancement of developers’ security aptitude.


2.1 Evolution of Vulnerability Detection Techniques

Vulnerability detection has evolved from traditional machine learning techniques to advanced deep learning-based solutions. As Lin et al. \cite{lin2020software} elucidate, while ML methods continue to be promising for automated vulnerability discovery, deep learning solutions like VulDeepecker \cite{li2018vuldeepecker} and μVulDeepecker \cite{zou2019mu} offer universal applicability but are heavily reliant on feature engineering.
In contrast, approaches like Devign \cite{zhou2019devign}, VulBERTa \cite{hanif2022vulberta}, and ReVEAL \cite{chakraborty2021deep}, utilize CPG-based [57] techniques for improved flexibility in vulnerability identification. AST-based proposed by Bilgin et al. \cite{bilgin2020vulnerability} and other \cite{lin2019software}, \cite{li2021towards}, \cite{dam2018automatic} and transformer-based models like RoBERTa \cite{liu2019roberta} were adopted by VulBERTa \cite{hanif2022vulberta} and \cite{thapa2022transformer} have also emerged, enhancing the retention of syntactic information and detection capabilities respectively. Lastly, Islam et al. \cite{islam2023unbiased} proposed a semantic understanding of programming languages to classify and detect vulnerabilities.

2.2 Source Code Vulnerability Localization

Various methods, from rule-based static analysis tools to innovative deep learning techniques, have been employed to localize source code vulnerabilities. Despite their direct approaches, tools like Cppcheck \cite{cppcheck}, FlawFinder \cite{flawfinder}, RATS \cite{rats}, and Infer \cite{infer} are criticized for their high false positive and negative rates \cite{yamaguchi2015pattern}  which raises the need for more reliable methods. 
A promising avenue is provided by the use of deep learning, as evidenced by the fine-grained vulnerability detection and locator systems proposed by Vuldeelocator \cite{li2021vuldeelocator} and DeepLineDP \cite{pornprasit2022deeplinedp}, leveraging Bidirectional Recurrent Neural Networks. Additionally, the ensemble graph transformer learning approach by VELVET \cite{ding2021velvet} and the non-conventional explainability technique by LineVul \cite{fu2022linevul} demonstrate advances in detecting and localizing vulnerabilities at the statement level. VulChecker \cite{mirskyvulchecker} presents a unique approach using an intermediate representation called LLVM for vulnerability localization. 


2.3 Root Cause Analysis Challenges and Solutions

Identifying the root cause of vulnerabilities is complex due to the disconnect between code crash states and actual root causes. Over time, several notable approaches have emerged. AutoPaG \cite{lin2007autopag}, for instance, leveraged the data flow of programs to analyze vulnerabilities such as out-of-bound, buffer overflow, and general boundary condition errors. To isolate the root cause of thread scheduling issues, Choi et al. \cite{choi2002isolating} proposed narrowing down differences in thread schedules, resulting in the program's failure. Further, Failure Sketching \cite{kasikci2015failure} introduced a cooperative adaptation of static and dynamic analysis for identifying root causes of production failures. More recent contributions, such as ARCUS \cite{yagemann2021arcus} and Yagemann et al.’s methodology {yagemann2021automated}, automate root cause analysis through execution flags and binary level analysis and tracking execution traces, respectively, enhancing the detection of issues like buffer overflow and use-after-free exploits.


2.4 Evaluating the Efficacy and Limitations of Contemporary Security Analysis Tools

The usability of various publicly available tools on code security is yet to be analyzed. Developers commonly use static analysis tools such as Infer \cite{infer} and Cppcheck \cite{cppcheck}, as well as deep learning methods [18] [34], to detect, localize [20] [35] [21], and repair [36] [37] vulnerabilities as we discussed earlier. These tools, while helpful, are not designed to be assistive or interactive in helping developers gain a comprehensive understanding of the vulnerabilities or the underlying reasons for their existence. Moreover, the risk of developers becoming overly reliant on these tools is evident, a scenario that contradicts the intended purpose of these resources. They are meant to serve as aids that enhance developers' security knowledge and competency in writing secure code, not replace the skillset altogether.


2.5 Development-Phase Vulnerability Analysis and Explainable Techniques

While the aforementioned methods focus on vulnerability analysis during a program’s execution, it is equally critical, from a developer’s perspective, to scrutinize vulnerabilities during the development phase \cite{islam2023unbiased} \cite{braz2022less}. This has led to the proposal of explainable techniques that pinpoint relevant features contributing to a program’s vulnerability \cite{mosolygo2021towards}, \cite{sotgiu2022explainability}, \cite{mao2020explainable}. Asm2Seq \cite{taviss2023asm2seq} and VulANalyzeR \cite{li2023vulanalyzer} took this concept further by introducing explainable deep learning-based approaches for identifying binary vulnerabilities in source code. Notably, VulANalyzeR \cite{li2023vulanalyzer} employed an attention-based explainable mechanism to unearth the root cause of vulnerabilities.


To conclude, we’ve explored various methods for vulnerability analysis, highlighting the shift towards development-phase vulnerability analysis and the use of explainable techniques. Our research aims to fill the gap in token-based vulnerability localization for C/C++ programming languages using large language models.







==> sections/Arezou_Survey_method_part.tex <==


\section{User-Focused Survey Design}
We designed a user-centric survey to evaluate our proposed system's effectiveness in addressing code vulnerability issues and aiding developers in learning secure coding practices without over-relying on AI tools. While our proposed system does not provide any code completions, we provided information to the developers to help them fix any possible vulnerability in their code. 
Our educational approach refrains from offering direct solutions. Instead, it equips developers with insights enabling them to address code vulnerabilities, ensuring they maintain full control over their code and its underlying logic. We tested our proposed system using undergraduate and graduate students from Computer Science with programming experience from an R1 research university.  



\subsection{Participant Recruitment}

We sourced our participants from the Computer Science department, enlisting both undergraduate and graduate students who have either completed or are currently enrolled in at least one programming language course. The recruitment process involved utilizing the students' mailing list, with the support of the department admin, to disseminate invitation emails.
Furthermore, since many of these participants will join the industry after graduation, their selection is strategic, considering they likely possess limited training in code security. This demographic allows us to gauge the ramifications of insufficient code security knowledge among emerging professionals.
We selected participants with a wide range of educational backgrounds: 1) Undergraduate Students with programming experience, 2) Graduate Students without industry experience, 3) Graduate Students with industry experience, and 4) Graduate Students with research Experience. 
The recruitment communication emphasized evaluating their code-writing quality, deliberately omitting the focus on code security practices. This omission aimed to prevent potential bias, as participants could have otherwise prepared in advance, skewing the results. 
Each participant received a compensation of \color{red} 25\$ for their contribution to the study. This study involved human participants and was approved by the institution’s Institutional Review Board (IRB).


\subsection{Procedure}
\color{red}
Do we need to justify, Why did we do it in C??? 
\color{black}

The study commenced with participants tackling programming tasks, each embedded with potential Common Weakness Enumeration (CWE) vulnerabilities. These tasks were designed in the C/C++ programming language to ensure consistency (what consistency?) in evaluation. Furthermore, we chose C/C++ as the programming language for our survey since many memory and resource-related vulnerabilities directly arise from it \cite{msrc}.

Participants were furnished with three types of information: 
1) the specific vulnerable line of code, a detailed description of the vulnerability category, 2) The vulnerability category and its description, and 3) an explanation of the root cause of the vulnerability. This approach contrasts with previous studies like PFGCN \cite{islam2023unbiased} and VulChecker \cite{mirskyvulchecker}, which, as discussed in Section \ref{1.5_motivation}, proved insufficient in empowering developers to rectify vulnerabilities autonomously and enhance their future code security practices.

For a nuanced understanding of our model's impact, participants were randomly allocated to two distinct groups: the Control Group and the Assisted Group. The control group was provided with the vulnerable line and its associated category. In contrast, the assisted group was also enlightened on the root cause of the vulnerabilities.
The control group imitates the current state-of-the-art methods, including assisting the developers by providing localization as the highest level of information. However, the assisted group imitates our proposed system, where the developers are provided with the root cause of the vulnerability and a description that helps them understand the vulnerability in the code.
We hypothesize that a clear comprehension of the vulnerabilities, supported by their classifications and detailed descriptions, will empower developers to amend the code adeptly, obviating the need for additional resources.



\subsection{Survey Design}

Our survey is structured in two distinct stages to rigorously evaluate the effectiveness of our model: the Learning Stage and the Evaluation Stage.

\textbf{Learning Stage:} 
Randomly assigned to the controlled or assisted groups, participants tackled 10 code vulnerability problems. The controlled group received vulnerability localization and classification, while the assisted group additionally gained insights into the root causes. We assume this division will cause some participants to learn and generalize code vulnerability better. After showing them the training codes, we provide the users with some exercise problems to understand how efficiently they are fixing vulnerabilities.


\textbf{Evaluation Stage:}
In this phase, we assess the participants' ability to apply and extend the knowledge they've acquired regarding the rectification of security-related code vulnerabilities. The assessment revolves around the same set of questions previously posed in Section \ref{1.5_motivation}. At this juncture, each participant is evaluated under the same criteria, irrespective of their initial grouping (controlled or assisted).
This stage is designed to gauge the participants’ capability to independently analyze and rectify code vulnerabilities without the assistance of AI tools information like classification, localization, or root cause.


\textbf{Coding Task}

Participants were tasked with completing ten C functions associated with a grocery store system. They downloaded a C source file containing skeletal code (i.e., a function declaration without implementation)for each function, accompanied by implementation instructions, parameter and return value details, and example usages. Participants were required to document the start and completion times for each function.

Given the focus of our survey on the security implications of unsafe code, we selected C as the study language. This choice stems from the ease of inadvertently introducing memory-related bugs in C, such as buffer overflows and null pointer dereferences. Languages like Java or Python handle such bugs differently, offering built-in safeguards and detection mechanisms. A basic understanding of C was a prerequisite for all participants.

The tasks involved core C programming concepts like file I/O and memory management, steering clear of advanced data structures. Figure \ref{fig:fig_3} illustrates one of the ten functions awaiting participant implementation. Essential C libraries and user-defined structures were supplied as depicted in Figure \ref{fig:fig_4}. Participants could consult online resources and utilize any text editor or IDE.

The initial function evaluates the possible combinations of purchasable items, designed to identify unintended stack or integer overflows and assess input validation. Functions 2-5 entail reading and writing to a newline-delimited file, which serves as the grocery store's database system. These tasks are susceptible to a range of vulnerabilities; however, they are designed to assess whether participants can adeptly open and close system resources, effectively load and retrieve contents from the file using a buffer, and allocate dynamic memory appropriately. 
The remaining functions (6-10) focus on user management within the store system, evaluating skills in string handling, array allocation/deallocation, and buffer length and capacity verification.
Participants are not provided assumptions or warned of potential edge cases to check for in any functions.



\color{black}


\subsubsection{Code Assessment}
We employed a dual-method evaluation approach to assess the participants' code, categorizing identified bugs according to their CWE classification \cite{cwe}.

\textbf{Run-time Analysis:} For the run-time of the code written by the participants, we generated two sets of test cases for each function. The first set aimed at evaluating the functionality, ensuring that the code meets the intended requirements. The second, more intricate set was designed to unveil potential vulnerabilities, with specific inputs crafted to induce run-time errors if vulnerabilities were present. A function passing all test cases was deemed free of vulnerabilities.

\textbf{Manual Analysis:} While most participants submitted a fully working code, some provided partially written non-compilable code. Furthermore, some participants also use pseudocode as a solution to vulnerability. Therefore, we also do a manual code review to identify potential vulnerabilities and fixes.


\color{black}


==> sections/backup.tex <==
\begin{table}[t]
\centering
\caption{Vulnerability Localization.}
\label{tab:rq1}
\begin{tabular} {p{0.14\textwidth}
                 p{0.1\textwidth}
                 p{0.08\textwidth}
                 p{0.08\textwidth}}
\toprule
\textbf{Model}                      & \textbf{Input}                          & \textbf{Dataset.}          & \textbf{Accuracy/IoU}  \\ \midrule
VELVET\cite{ding2021velvet}             & Token                          & D2A &  30       \\

VulDeeLocator \cite{li2021vuldeelocator}               & Slice + Token & NVD         & 17.68 \\

LineVul \cite{li2021sysevr}                    & Token                               & Big-Vul         & 24.46    \\
RoBERTa (Ours)                      & Token                            & Big-Vul         &  52.6        \\

RoBERTa (Ours)                      & Token                            & D2A         & 53.1         \\
\bottomrule


%\textbf{RoBERTa-GCN w/ WL} & Semantic Vulnerability Graph                 & 88.07         &46.34          & 49.14         & 47.31 \\
%\textbf{RoBERTa-GCN w/ FL} & Semantic Vulnerability Graph       & 89.88 & \textbf{57.52} & \textbf{50.20} & \textbf{47.91}     \\ \bottomrule


\end{tabular}
\end{table}




Since we are proposing a novel token-based vulnerability localization system, we compare our work with the recent baselines as follows.


\begin{itemize}
    \item BiLSTM \cite{hochreiter1997long}: Is a standard model for text/code classification or localization. BiLSTM accounts the long-term relationship among the tokens of a program.

    \item CodeBERT \cite{feng2020codebert} Its a BERT \cite{devlin2018bert} based model pretrained on 6 programming languages (Python, Java, JavaScript, PHP, Ruby, Go) using masked language modeling technique.

    \item GraphCodeBERT \cite{guo2020graphcodebert} Is a new pre-trained PL model that was trained using C/C++ that extends CodeBERT by taking the intrinsic structure data flow into the training objective.

    \item Devign \cite{zhou2019devign} Devign takes CPG as input and maintains the original of graph using a Graph Neural Network during training.
\end{itemize}



\begin{figure}[b]
    %\begin{framed}
        \centering
        
        \includegraphics[width=0.5\textwidth]{images/comparison_1.pdf}
        
    %\end{framed}
    \caption{Causality analysis of Vulnerability by comparing Attention and SHAPly values}
    \label{fig:fig_5}
\end{figure}




% Threats to validity(1)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering

\begin{tabular} {p{0.12\textwidth}
                 p{0.10\textwidth}
                 p{0.01\textwidth}}


\hline
\textbf{Model}    & \multicolumn{1}{l}{\textbf{Big-Vul}} & \multicolumn{1}{l}{\textbf{D2A}}  \\ \hline

\multirow{1}{*}{RoBERTa-GCN}   & \textbf{0.47} & \textbf{0.58}\\
            
                       
                       \hline
\multirow{1}{*}{RoBERTa} & 0.45 & 0.56 \\
                       
                       \hline
\multirow{1}{*}{GCN} & 0.46 & 0.57\\
                       
                       \hline



\end{tabular}
\caption{10 Fold Cross-Validation on the two Datasets}
\label{tab:crossval}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure}[htb]
    \begin{framed}
        \centering
        \begin{subfigure}[b]{0.49\textwidth}
            %\centering
            \includegraphics[width=1\columnwidth]{images/ex_shap_1.pdf}%\vspace{-0.5cm}
            %\caption{1}
            \label{fig:white1}
            \includegraphics[width=1\columnwidth]{images/comparison_2.pdf}
            %\caption{3}
            \label{fig:white2}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.5\textwidth}
            %\centering
            \includegraphics[width=1\columnwidth]{images/comparison_1.pdf}
            %\caption{2}
            \label{fig:white2}
        \end{subfigure}

    \end{framed}
    \caption{Q-Learning based Reinforcement Learning results. Reward ((a) Reward 5 and (b) Reward 6) and K(safe) values based on RB and GC over Time}
    \label{fig:rl_r1_vs_r2}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{table}[t]
\centering
\caption{Vulnerability classification with Big-Vul and D2A dataset using our proposed Ensemble RoBERTa GCN. \color{red} }
\vspace{0.3cm}
%\begin{tabular}{@{}cccccc@{}}
\begin{tabular}{p{0.10\textwidth}
                 p{0.45\textwidth}
                 p{0.08\textwidth}
                 p{0.08\textwidth}
                 p{0.08\textwidth}
                 p{0.08\textwidth}}
\toprule
\textbf{Data}                           & \textbf{Model}                              & \textbf{Acc.}            & \textbf{F1}      & \textbf{Pre.}         & \textbf{Rec.}                  \\ \midrule



\multirow{2}{*}{D2A}           & VELVET \cite{ding2021velvet}        & 0.59  & 0.58  &\textbf{0.70}  & 0.50        \\
                               & \textbf{Ensemble RoBERTA and GCN}         & \textbf{0.60}    & \textbf{0.68} & 0.58          & \textbf{0.82}\\ 
\toprule
\multirow{6}{*}{BigVul} & LineVul \cite{fu2022linevul}     & -          & 0.91              & \textbf{0.97}              & 0.86              \\

    & IVDetect \cite{li2021vulnerability} & -          & 0.35          & 0.23          & 0.72          \\
    & ReVEAL \cite{chakraborty2021deep}  & -          & 0.30          & 0.19          & 0.74          \\
    & Devign \cite{zhou2019devign}  & -          & 0.26          & 0.18          & 0.52          \\
    & \textbf{Ensemble RoBERTA and GCN}         & \textbf{0.63} &  \textbf{0.92} & 0.96 & \textbf{0.87} \\

                               
\bottomrule
\end{tabular}


\label{tab:class}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[b]
\centering
\caption{Vulnerability Localization using D2A and Big-Vul Dataset. We used two pre-processing techniques of code: SVG and AST}
\vspace{0.3cm}
\begin{tabular} {p{0.14\textwidth}
                 p{0.35\textwidth}
                 p{0.18\textwidth}
                 p{0.18\textwidth}}


\hline
\textbf{Input}    & \multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{l}{\textbf{IoU(SVG)}} & \multicolumn{1}{l}{\textbf{IoU(AST)}} \\ \hline
\multirow{5}{*}{D2A}   & Devign & 0.58 & 0.07 \\
%                       & RoBERTa & 0.42 & 0.09 & 0.41 \\
%                       & GCN & 0.58 & 0.06 & 0.43 \\
                       & VELVET &  0.55 & 0.09  \\
                       & LineVul & 0.42 & 0.06  \\
                       & \textbf{Ensemble RoBERTA and GCN} & \textbf{0.61} & 0.08 \\
                       \hline
\multirow{5}{*}{Big-Vul} & Devign & 0.44 & 0.06 \\
%                       & RoBERTa &  0.45 & 0.09 & - \\
%                       & GCN & 0.44 & 0.07 & - \\
                        & VELVET & 0.45 & 0.09 \\
                        & LineVul & 0.45 & 0.07  \\
                        & \textbf{Ensemble RoBERTA and GCN} & \textbf{0.49} & 0.07  \\ \hline



\end{tabular}

\label{tab:locz}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ablation Backup
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\caption{Ablation study on the contribution of each models}
%\vspace{0.3cm}
%\begin{tabular}{@{}cccccc@{}}
%\begin{tabular}{p{0.04\textwidth}
%                 p{0.08\textwidth}
%                 p{0.04\textwidth}
%                 p{0.04\textwidth}
%                 p{0.04\textwidth}
%                 p{0.04\textwidth}
%                 p{0.04\textwidth}}

\begin{tabular}{@{}clllllll@{}}

\toprule
\multicolumn{1}{l}{\textbf{Dataset}} & \textbf{CodeT5} & \textbf{GCN}  & \textbf{IoU} & \textbf{Acc}  & \textbf{F1}   & \textbf{Pre.} & \textbf{Rec.} \\ \midrule
\multirow{5}{*}{D2A}        & 0.20   & 0.80 &     & \textbf{0.65} & 0.49 & 0.57 & \textbf{0.65} \\
                            & 0.40   & 0.60 &     & 0.61 & 0.54 & 0.58 & 0.60 \\
                            & 0.60   & 0.40 &     & 0.60 & 0.59 & 0.59 & 0.60 \\
                            & 0.80   & 0.20 &     & 0.59 & 0.46 & 0.53 & 0.59 \\ 
                            & 0.50   & 0.50 &     & 0.60 & \textbf{0.69} & \textbf{0.60} & 0.61 \\
                            \midrule
\multirow{4}{*}{BigVul}     & 0.20   & 0.80 &     & \textbf{0.71} & 0.59 & 0.55 & \textbf{0.71}    \\
                            & 0.40   & 0.60 &     & 0.66 & 0.62 & 0.61 & 0.66    \\
                            & 0.60   & 0.40 &     & 0.63 & 0.61 & 0.61 & 0.63    \\
                            & 0.80   & 0.20 &     & 0.62 & 0.60 & 0.61 & 0.62    \\
                            & 0.50   & 0.50 &     & 0.65 & \textbf{0.64} & \textbf{0.62} & 0.65    \\ \bottomrule
\end{tabular}


\label{tab:abl_1}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\vspace{-3mm}
\subsection{Effectiveness of Combined Learning Ensemble Model}

To demonstrate the superiority of our ensemble model, we built and tested our models using RoBERTa or GCN only for comparison. Our experimental results in Table \ref{tab:crossval} indicate that for vulnerability localization, the IoU value increases by up to 5\% compared to using GCN or RoBERTa alone. Additionally, we observe a 4\% increase in the F1 score for the vulnerability classification task. Thus, our ablation study confirms that our ensemble model outperforms in both vulnerability classification and locating the vulnerable line.

\color{red}

\subsection{Importance of Individual Embedding Generated by Our Ensemble Model}
The goal of an ensemble model is to combine several individual models to achieve superior performance. The ability to bring diverse data to fit into a model shows the diverse capabilities of an ensemble model. Therefore, in our training and inferencing step, we took the average embedding generated from CodeT5, $F_R$, and GCN $F_{GCN}$.

However, in our dataset, there is a good mix of different categories of vulnerabilities, some of which are more easily detectable by a GCN model and some using transformers. Therefore to understand how each model contributes to the detection and localization capability of our model, we multiply the embedding with varying constants $\kappa$ and $\lambda$. 

\begin{equation}
    \label{eqn:12}
    F_E = \kappa \times F_R + \lambda \times F_{GCN}
\end{equation}

We vary the value of $\kappa$ and $\lambda$ from 0 to 1, such that their sum is always 0. When the value of $\kappa$ is lower compared to $\lambda$, we see an increase in performance, indicating that $F_{GCN}$ has more effect on the performance since the majority of embeddings are coming from both the datasets. When any of the value of $\kappa$ or $\lambda$ is zero, it is equivalent to not using the model at all for classification and localization purposes.

\color{blue}
From Table \ref{tab:abl_1}, we can see that the although we see higher accuracy with 20:80 of CodeT5 and GCN, we see a significant drop in F1 scores for this case in both D2A and BigVul datasets. We also observe that when the ratio goes close to 1, there is an improvement in the F1 scores, and when the ratio is 50:50, we achieve the highest F1 scores concluding the effectiveness of our ensemble model.  

We further investigated the outcome of multiclass vulnerability detection and compared the F1 scores of the ensemble models when the model's different ratios were considered. From Figure \ref{fig:chart_abl}, we can see a distinction among the F1 scores of each class. For some CWE classes like CWE-119, CWE-20, CWE-125, and CWE-189, we see an upward trend in the F1 scores than the contribution of the GCN model is higher. This also explains that these vulnerabilities are memory-related and hence can be easily detectable by the GCN model. However, for the rest of the vulnerabilities, we see a downward trend when the contribution of CodeT5 is lessened, concluding the effectiveness of CodeT5 in classifying these vulnerabilities. This also explains higher accuracy, although lower F1 scores when we use the 20:80 ratio on the ensemble model.

\color{black}

\begin{figure*}[t]
    %\begin{framed}
        \centering
        
        \includegraphics[width=0.8\textwidth]{images/ablation_chart.pdf}
        
    %\end{framed}
    
    \caption{Multiclass classification of vulnerability by varying the contribution of each component of our ensemble model}
    \label{fig:chart_abl}
\end{figure*}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\centering
\caption{Ablation study on the Contrubution of each model}
%\vspace{0.3cm}
%\begin{tabular}{@{}cccccc@{}}
\begin{tabular}{p{0.04\textwidth}
                 p{0.08\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}}
\toprule
\textbf{Data} & \textbf{Model} &\textbf{IoU}  &\textbf{Acc.} & \textbf{F1} & \textbf{Pre.} & \textbf{Rec.} \\ \midrule



\multirow{3}{*}{D2A}           & GCN   & 0.52     & 0.59  & 0.58  &\textbf{0.70}  & 0.50        \\                          
                               & RoBERTA   & 0.53      & 0.54    & 0.64 & 0.56          & 0.80\\
                               
                               & \textbf{Ensemble(Ours)}   & \textbf{0.57}      & \textbf{0.60}    & \textbf{0.68} & 0.58          & \textbf{0.82} \\
\toprule
\multirow{3}{*}{BigVul} & GCN  & 0.39    & 0.58          & 0.91              & \textbf{0.97}              & 0.86              \\

    & RoBERTa & 0.42 & 0.60          & 0.88          & 0.90          & 0.80          \\
    & \textbf{Ensemble(Ours)}   & \textbf{0.46}      & \textbf{0.63} &  \textbf{0.92} & 0.96 & \textbf{0.87} \\

                               
\bottomrule
\end{tabular}


\label{tab:ablation_2}
\end{table}

\color{black}


\subsection{Ablation of Root Cause analysis through explainability}

In order to compare our root cause of vulnerability analysis technique using DeepLiftShap, we also use an in-build property of the transformers called the attention values. The attention score evaluates the strength of a token's relationship with the other words in the sequence, providing a causal relationship between two tokens. The Self-Attention layer in each encoder generates an attention value for each token, which is learned during training. We extract the values from all the attention heads into a single vector, thus getting equivalent scores for each line. However, attention values do not have a lower and upper limit than the DeepLiftShap scores. Therefore, after getting attention scores for all the lines, we convert them between the range of 0 to 1 to properly compare attention scores and DeepLiftShap.

Our analysis in Figure \ref{fig:cs_a} shows that, although in this example, we were able to determine localization for functions with a smaller number of lines, the attention values fluctuate more frequently, as we can see from the values for line 6, 7 and 8. Similarly, in the root cause analysis in the yellow highlighted part, the value changes more frequently. Another interesting observation on the attribution score is that the attention values in the first line and comparatively high in this sample, whereas the DeepLiftShap value is relatively small. This indicates that the attention-based model incorrectly predicts a line as the root cause. Line 1 is the declaration line of a function; hence, it can be neither a vulnerable line nor a line that is the root cause of a vulnerability.


\begin{figure}[t]
    %\begin{framed}
        \centering
        
        \includegraphics[width=0.5\textwidth]{images/case_study_ablation.pdf}
        
    %\end{framed}
    
    \caption{An ablation study on the comparison of }
    \label{fig:cs_a}
\end{figure}

\color{black}



\subsection{Ablation study on Localization Using Generative Approach}

Since a part of our ensemble model is a CodeT5 transformer with an encoder and a decoder, we further test the localization capability of our model using the generative capability of the transformer. Therefore, instead of using the ensemble approach, we use the CodeT5 transformer to generate the vulnerable statement in the source code. Thus, we trained the transformer to generate the vulnerable state using the cross-entropy loss function. However, our ensemble approach is the token range of the vulnerable lines, and this approach generates the entire vulnerable statement. Therefore to have a fair comparison, we convert the token range into line(s) by locating which line the token range exists. We also convert the generated statement by the transformer model into its corresponding lines. After we have the generated lines from the ensemble model and output from the transformer model, we compare them. If the lines have matches exactly, we render them as an exact match (EM). 

Generative models, however, sometimes produce garbage output, and therefore it is impossible to map some outputs of the generative model to the actual input code. We consider these cases unmatched and with an EM value of 0.

Table \ref{tab:abl_3} shows the EM values for each dataset. We see that the exact match for the Generative CodeT5 on D2A is 56\%  percent, while the exact match for our ensemble model is 75\%, almost a 15\%  improvement, indicating our model's superiority. For the BigVul dataset, we also see a 12\% improvement. Furthermore, we also tested each component of our ensemble model, and in all the cases, we saw a significant improvement in results using our token-based approach.  



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[t]

\centering
\caption{Ablation study on vulnerability localization with generate model}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Dataset} & \textbf{D2A} & \textbf{BigVul} \\ \midrule
CodeT5 (Encoder) &  0.55    &    0.40   \\
GCN  &  0.63    &   0.46    \\
Generative CodeT5  &     0.60       &   0.41  \\ 
Ensemble (Ours)     &     0.75       &   0.53   \\
\bottomrule
\end{tabular}
\label{tab:abl_3}
\end{table}






\color{black}


%In order to show that our ensemble model works better, we build a model using only RoBERTa or GCN. Our experimental results from Table \ref{tab:crossval} shows that for vulnerability localization, the IoU value has increased up to 5\% compared with GCN or RoBERTa. We also see an F1 score increase of 4\% for the vulnerability classification task. Hence our ablation study concludes that our ensemble model performs better in vulnerability classification and finding the vulnerable line.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ablation Backup Done
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[b]
\centering
\caption{Ablation study on the contribution of each component of the ensemble model}
%\vspace{0.3cm}
%\begin{tabular}{@{}cccccc@{}}
%\begin{tabular}{p{0.04\textwidth}
%                 p{0.08\textwidth}
%                 p{0.04\textwidth}
%                 p{0.04\textwidth}
%                 p{0.04\textwidth}
%                 p{0.04\textwidth}
%                 p{0.04\textwidth}}

\begin{tabular}{@{}clllllll@{}}

\toprule
\multicolumn{1}{l}{\textbf{Dataset}} & \textbf{CodeT5} & \textbf{GCN}  & \textbf{IoU} & \textbf{Acc}  & \textbf{F1}   & \textbf{Pre.} & \textbf{Rec.} \\ \midrule
\multirow{5}{*}{D2A}        & 0.20   & 0.80 & 0.69 & \textbf{0.65} & 0.49 & 0.57 & \textbf{0.65} \\
                            & 0.40   & 0.60 & 0.68 & 0.61 & 0.54 & 0.58 & 0.60 \\
                            & 0.60   & 0.40 & 0.65 & 0.60 & 0.59 & 0.59 & 0.60 \\
                            & 0.80   & 0.20 & 0.67 & 0.59 & 0.46 & 0.53 & 0.59 \\ 
                            & 0.50   & 0.50 & \textbf{0.72} & 0.62 & \textbf{0.68} & \textbf{0.60} & 0.65 \\
                            \midrule
\multirow{4}{*}{BigVul}     & 0.20   & 0.80 & 0.46 & \textbf{0.71} & 0.59 & 0.55 & \textbf{0.71}    \\
                            & 0.40   & 0.60 & 0.46 & 0.66 & 0.62 & 0.61 & 0.66    \\
                            & 0.60   & 0.40 & 0.44 & 0.63 & 0.61 & 0.61 & 0.63    \\
                            & 0.80   & 0.20 & 0.45 & 0.62 & 0.60 & 0.61 & 0.62    \\
                            & 0.50   & 0.50 & \textbf{0.49} & 0.65 & \textbf{0.64} & \textbf{0.62} & 0.66    \\ \bottomrule
\end{tabular}


\label{tab:abl_1}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%   Generalizability Testing %%%%%%%%%%%%%%

\textbf{Generalizability Testing:} We test our model's generalizability by testing the model's outcome on IoT device operating systems. To achieve this, we trained our model with one dataset and tested the model’s performance on a different dataset to observe our model’s generalization efforts. Furthermore, to achieve more generalizability, we combined both the D2A and BigVul dataset and tested the model's performance. When we trained the model on the D2A dataset and tested it on the BigVul dataset and vice versa, we can see from Table \ref{tab:generaility} that the accuracy has decreased. However, when we trained the model with the combined dataset, we see that the F1 scores had increased up to 7\% and the IoU score had increased by 2\% for D2A dataset. Moreover, the IoU score has increased 1\% for BigVul Dataset. We observe that when we use the combined dataset for training, metrics for D2A increase significantly since D2A dataset is 26 times smaller than BigVul, hence providing more generalizability to our model.



\begin{table}[t]
\centering
\caption{Generalizability Testing of our Model. We test with out-of-sample data during evaluation to test the generalizability of the model}
%\vspace{0.3cm}
\label{tab:generaility}
\begin{tabular}{p{0.07\textwidth}
                 p{0.07\textwidth}
                 p{0.03\textwidth}
                 p{0.03\textwidth}
                 p{0.03\textwidth}
                 p{0.03\textwidth}
                 p{0.04\textwidth}}
\toprule
\textbf{Training Data} & \textbf{Evaluation Data} & \textbf{IoU} &\textbf{Acc.} & \textbf{F1} & \textbf{Pre.} & \textbf{Rec.}      \\ \midrule

\multirow{2}{*}{D2A} & D2A & 0.72 & 0.62  & 0.68  &0.68  & 0.65   \\
                                    & BigVul & 0.40 & 0.52  & 0.55  &0.57  & 0.52 \\ \midrule
                                                    
\multirow{2}{*}{BigVul} & BigVul & 0.49 & 0.65  & 0.62  &  0.66  & 0.66     \\
                                    & D2A & 0.44 & 0.57  & 0.59  &0.60  & 0.51 \\ \midrule
                                    
\multirow{3}{*}{D2A+BigVul} & D2A & 0.74 & 0.66  & 0.75  &0.70  & 0.70     \\

& BigVul & 0.50 & 0.64  & 0.66  &0.67  & 0.70 \\

& D2A+BigVul & 0.65 & 0.68  & 0.64  &0.66  & 0.69 
                                    
%\vspace{-5mm}                                  
\\\bottomrule



\end{tabular}
\end{table}





% Overall challenges with these tools: --> leads to root cause
% Does not connect with previous paragraph
While these currently available techniques provide some security, they fail to deliver a usable code security system that helps developers write and understand code security issues during development. While vulnerability classification and localization play a critical role in discerning the specific location of code failure, it cannot determine the root cause of the vulnerability. This problem is further exacerbated within large-scale applications, potentially comprising millions of lines of code, where crash reproduction can be exceptionally challenging due to environmental discrepancies \cite{bellare1997forward}, \cite{capobianco2019employing} \cite{han2020unicorn} of the system. Although capturing program stack traces or logs \cite{ji2017rain} \cite{kang2011dta} might provide insights such as vulnerability-causing inputs or code break locations, the derived results are often incomplete as they do not necessarily identify the root cause of the vulnerability. While tainting \cite{ji2017rain} \cite{slowinska2007age} and replaying \cite{196257} \cite{268240} techniques may assist developers in uncovering code vulnerabilities, the identification of the specific code block instigating the vulnerability \cite{yagemann2021arcus}  would be of paramount benefit. 

%Our proposed system is the first to integrate an IoT operating systems repository scanner for function extraction using Joern \cite{joern} and a large language model VulCodeT5 to generate descriptions for the developers in repairing vulnerabilities. 

To address these challenges, we are the first to introduce VulCodeT5, a large language model for vulnerability localization and causative insights into the vulnerability. Our proposed VulCodeT5 provides GCN \cite{kipf2016semi} architecture powered by a CodeT5 embedding \cite{wang2021codet5} for vulnerability classification and localization, which harnesses the sequential/syntactical structure of tokens and the graphical structure of a programming language, respectively. Furthermore, we incorporate an explainability-based method to extract the relationship between a vulnerable statement and the statement most contributing to the vulnerability's root cause. The efficacy of our system is substantiated through an exhaustive case study analysis, focusing on evaluating 1) the model's classification performance and vulnerable line detection, 2) the effect of the outcome on the developers in writing secure code, and 3) demonstrating the application of our system by identifying the root cause analysis of vulnerability and its ability to identify and localize N-day and zero-day vulnerabilities in the wild.



-------------------- Original Survey Portion Written by Nafis --------------------




\subsection{User-Focused Survey Design}

\subsubsection{Overview} 

Our user-focused survey aims to determine the impact of our proposed system in resolving code vulnerability and its aid on developers in learning how to write secure code without being excessively dependent on AI-assisted tools. While our proposed system does not provide any code completions, we provided information to the developers to help them fix any possible vulnerability in their code. 


In order to educate the developers intuitively, we do not provide any solutions to the developer; instead, we provide helpful insights about code, which helps them fix the vulnerability of code while keeping the developers in control of their code and business or program logic. 

We examined our system's outcome by leveraging undergraduate and graduate students' knowledge in software development from an R1 research university. 

We recruited the participants by advertising them through the department admins and social media. The participants were asked about programming tasks initially. Each of the programming tasks has the possibility of a particular CWE vulnerability category. All the programming assignments are written in C/C++ programming language.


We provided three types of information to our participants: 1) The localized vulnerable line, 2) The vulnerability category and its description, and 3) The root cause of the vulnerability. Prior works like PFGCN \cite{islam2023unbiased} and VulChecker \cite{mirskyvulchecker} provide this information. However, Section \ref{1.5_motivation} demonstrates that these methods are not enough to solve the vulnerability, as they don't help the developers write more secure code in the future.

To understand the effect of our model's three pieces of information, we randomly divided the participants into two groups: 1) Control group, and 2) Assisted Group. The control group was provided with two pieces of information: the localized vulnerable line and its category. However, we provided the assisted group with three types of information we mentioned above.  The control group imitates the current state-of-the-art methods, including assisting the developers by providing localization as the highest level of information. However, the assisted group imitates our proposed system, where the developers are provided with the root cause of the vulnerability, which helps them understand the vulnerability in code. In this learning phase, we hypothesize that if the developers are clear about the reasoning behind the vulnerability with proper classification and description, they can fix the code without any external knowledge.

\subsubsection{Participant Recruitment}

We recruited undergraduate and graduate students from the Computer Science department who have taken at least one programming language course or are currently taking a programming language course. We recruited students from the students' mailing list and sent them invitation emails with the help of the Computer Science department admin. Furthermore, since many of these participants will join the industry after graduation, they are perfect participants because they are less likely to be trained in code security, and the impact of leaving out code security can be understood.

We selected participants with a wide range of educational backgrounds: 1) Undergraduate Students with only programming experience, 2) Graduate Students without industry experience, 3) Graduate Students with industry experience. During recruitment, we only stated that we would test the participants' code-writing quality. However, we did not mention that we would evaluate the code security practice of students because they may have prepared about code security before participation, which would make our analysis biased. We provided a compensation of \color{red} X\$  to each participant to participate in the survey. This study involved human participants and was approved
by the institution’s Institutional Review Board (IRB). \color{black}


\subsubsection{Workflow of the Survey}

Our survey consists of 2 stages to analyze the outcome of our model. First is the learning stage, and second one is the evaluation stage.

\textbf{Learning Stage:} In the learning stage, we split the participants randomly into two groups, controlled and assisted. We provided 10 specially crafted code vulnerability problems to the participants. The controlled group was the provider with localization and classification of vulnerability and the assisted groups were provided the two prior information, with the addition of root cause of the vulnerability. We assume this division will cause some participants to learn and generalize code vulnerability better. After showing them the training codes, we provide the users with some exercise problems to understand how efficient they are with fixing vulnerabilities.

These exercise problems are similarly divided among the participants. The controlled group will have only access to 2 information, and the assisted group will have access to 3 information. Based on how much the participants can solve the code's vulnerability, we test our system's efficiency as an assisted tool that can help developers fix a vulnerability.


\textbf{Generalization Stage:} This stage aims to determine how the developers have generalized their knowledge of fixing security-related source code vulnerabilities. Therefore, we ask them the same question we asked them before in \color{red} Section \ref{1.5_motivation}.\color{black} However, in this case, we do not differentiate any questions or problems regardless of the participant's controlled or assisted category. We ask the participants to reevaluate their code based on what they learned at the evaluation stage. This time, we do not provide any AI-assisted service like classification, localization, or root cause. We aim to find how self-sufficient the developers are in writing secure code without assistance and how efficiently they can solve the vulnerability.

\lstinputlisting[style=CStyle, label={lst:lst1}, caption=One of the C functions to be completed by the participant. The skeletal code outlines the implementation instructions\, example usage\, parameter and return value documentation\, and time started and completed indicators.]{code/problem2.c}

\subsubsection{Programming Assignment}

\textbf{Summary}: The participants were instructed to complete 10 C functions related to a grocery store system. Specifically, the participants were instructed to download a C source file containing "skeletal code" (i.e., a function declaration without implementation) of 10 functions, with each function containing documentation on the function's implementation instructions, parameter and return value information, and example usage. The participants were instructed to complete one function at a time and to document the time they began and finished each function.

\textbf{C Language Study}: Our survey concerns the security consequences of unsafe code. Therefore, we chose C as our study language due to the numerous amounts of memory-related bugs that may be quickly introduced in C code unknowingly by software developers. Memory-related bugs, such as buffer overflows and null pointer dereferences, have different consequences in languages like Java or Python. These languages have built-in measures to mitigate the damage and make it easier to detect such bugs through exception handling and compiler checks. All study participants were expected to have a basic understanding of the C programming language to participate in our survey.

\textbf{Instructions}: The C source code file contains instructions for the participants at the top of the file. It specifically asks participants to read the instructions of each function carefully, complete one function at a time, and document the time they began to code each function and the time they were done coding each function. Participants were not prohibited from using any online resource or large language model to help them with writing their code, and they were allowed to use any text editor or integrated development environment of their choice.

\textbf{Implementation Details}: All ten functions the participants implemented only incorporate basic C concepts such as file I/O reading and writing and memory management. Participants were provided with basic C libraries, and some simple user-defined structures seen in Listing \ref{lst:lst2}. This survey does not incorporate data structure concepts such as linked lists and binary search trees. Listing \ref{lst:lst1} is one of the ten functions the participant is required to complete, with the function documentation clearly outlining the implementation instructions, example usage, and comments indicating where the participant should mark the time they started to implement the function and the time they completed implementing the function.

The first function involves calculating the number of possible combinations of items a customer can buy. The design of this problem is to check if the participant unknowingly introduced a stack overflow or integer overflow and ensure they validated the input argument. Functions 2 through 5 involve reading and writing to a newline delimited file representing the grocery store database system. A variety of vulnerabilities can accidentally be introduced in these problems, but the design of these problems is primarily to check if the participant opened and closed system resources correctly, loaded the contents to and from the file using a buffer, and dynamically allocated memory appropriately. Functions 5 through 10 involve managing users of the grocery store system. The design of these problems includes string handling, correct array allocation and deallocation using a user-defined data type, and verifying buffer length and capacity.

Participants are not provided any assumptions or warned of potential edge cases to check for in any functions.



\lstinputlisting[style=CStyle, label={lst:lst2}, caption=The included headers\, defined constants\, and defined structures used in the survey.]{code/survey_assumptions.c}

\lstinputlisting[style=CStyle, caption=A function that primarily checks if the participant properly deallocated an array.]{code/problem5.c}





\color{black}



\subsubsection{Evaluation of Code:}
We used two types of evaluation in order to test the code written by the participants. Each of the identified bugs were categorized into their CWE \cite{cwe} category.

\textbf{Run-time Analysis:} For run-time of the code written by the participants, we generated some test-cases for each of the functions. For each function, there are two sets of test cases. The first set of test cases are for functionality testing of the given functions. The second set of test cases are tricky test cases. Based on the input in the test cases of this set, if there is a run-time error in code, it demonstrates the existence of a particular vulnerability in that code. If a function passes all the test cases, we consider the function as vulnerability free.

\textbf{Manual Analysis:} While most of the participants submitted a fully working code, some provided partially written code that are non compilable. Furthermore, some participants also pseudocode as a solution to vulnerability. Therefore, we also do a manual code review to identify potential vulnerabilities and fixes.


\lstinputlisting[style=CStyle, caption=A function that primarily checks if the participant handled adding an element to an array correctly (with a simplified comment block.)]{code/problem7.c}

\color{black}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Technical challenges with these tools
At the same time, recent user-focused research suggests that software developers need critical support when addressing security challenges \cite{acar2016you, green2016developers}. While for code analysis, static or rule-based methods exist \cite{shin2010evaluating, engler2001bugs} for source code vulnerability detection and classification \mj{this sentence is unclear!}. Static analysis tools like FlawFinder \cite{flawfinder} and Cppcheck \cite{cppcheck} endeavor to categorize and localize vulnerabilities using these rule-based strategies; however, they are challenged by high false positives and false negatives rates \cite{yamaguchi2015pattern}. On top of these limitations, the lack of proper recommendations for developers on solving vulnerability has catalyzed the utilization of sophisticated deep-learning vulnerability detection \cite{russell2018automated, zhou2019devign}. Similarly, localization methods \cite{ding2021velvet, fu2022linevul, mirskyvulchecker}, which significantly alleviate developers' burden by providing them with invaluable information to rectify vulnerabilities however, are challenged with easiness of the understandability of developers why a particular vulnerability was flagged \mj{this sentence is unclear and needs re-write!}.

% Overall challenges with these tools: --> leads to root cause: recommentadion
% Does not connect with previous paragraph
%While these currently available techniques provide some security, they fail to deliver a usable code security system that helps developers write and understand code security issues during development. 

\mj{Combine multiple citations into a single $\backslash$ cite tag!} While vulnerability classification and localization play a critical role in discerning the specific location of code failure, it cannot determine the root cause \cite{mirskyvulchecker} of the vulnerability. This problem is further exacerbated within large-scale applications, potentially comprising millions of lines of code, where crash reproduction can be exceptionally challenging due to environmental discrepancies \cite{bellare1997forward, capobianco2019employing, han2020unicorn} of the system. Although capturing program stack traces or logs \cite{ji2017rain, kang2011dta} might provide insights such as vulnerability-causing inputs or code break locations, the derived results are often incomplete as they do not necessarily identify the root cause of the vulnerability. Consequently, these run-time analyses from stack traces are after the entire deployment application, which is highly time-consuming and, at the same time, causes too much back and forth between code writing and full deployment. While tainting \cite{ji2017rain, slowinska2007age} and replaying \cite{196257, 268240} techniques may assist developers in uncovering code vulnerabilities, the identification of the specific code block instigating the vulnerability \cite{yagemann2021arcus}  would be of paramount benefit. 
 




















==> sections/introduction_BK.tex <==


--------- Backup of the introduction ------------------


%The proliferation of dangerous cyberattacks around the globe has disrupted the Open Source Software (OSS) industry heavily and  cause widespread downstream detrimental effects. Moreover, OSS plays a vital role across a government and its infrastructure vulnerabilities in open-source software components may cause widespread downstream detrimental effects \cite{synopsysrisc}. Following the aftermath of Log4Shell \cite{log4j} an interagency working group Open-Source Software Security Initiative (OS3I) was formed with the goal to integrate agencies like Cybersecurity Infrastructure Security Agency (CISA), the National Science Foundation (NSF), Defense Advanced Research Projects Agency (DARPA), National Institute of Standards and Technology (NIST) to work colaboratively with the mindsed to identify OSS security priorities and policies \cite{fedreg}. 

%Moreover, OSS plays a vital role across a government and its infrastructure vulnerabilities in open-source software components may cause widespread downstream detrimental effects \cite{synopsysrisc}.

%Moreover, vulnerabilities in OSS plays a vital role across a government and its infrastructure causing widespread downstream of detrimental effects \cite{synopsysrisc}.

%\color{red}

% General Challenge of Cyberattack on Code

In an era of escalating cyber threats, the Open Source Software (OSS) community stands at an unprecedented crossroads, charged with safeguarding the very foundation of countless software systems and products integral to modern society.
%The escalating frequency of severe cyberattacks on a global scale has disrupted the Open Source Software (OSS) community significantly, causing widespread downstream detrimental effects. 
Nevertheless, security vulnerabilities in poorly written software play a vital role across government and its infrastructure, causing widespread disruption of services\cite{synopsysrisc}. In the aftermath of the Log4Shell incident \cite{log4j}, an interdisciplinary consortium, the Open-Source Software Security Initiative (OS3I), was formed to mobilize agencies such as the Cybersecurity Infrastructure Security Agency (CISA), National Science Foundation (NSF), Defense Advanced Research Projects Agency (DARPA), and National Institute of Standards and Technology (NIST) to delineate software security priorities and formulate cohesive policies collaboratively \cite{fedreg}. %Whether it is open-source or not, code security in a software ecosystem is a paramount concern that demands rigorous attention, concerted efforts, and innovative solutions for private entities and large enterprises.

%enabling more people to engage in 
The landscape grows more intricate with emerging technologies like ChatGPT, which despite enhancing developers' coding ability, introduces significant security challenges.
%While OSS and the recent advent of ChatGPT have accelerated the programming capabilities of developers, it has brought some security challenges 
\cite{khoury2023secure, sandoval2022security}. Open source code being highly accessible, novice developers are likely to use this code to complete the functionality of their coding task. Although this democratization of coding has increased the developers' productivity by enabling more people to engage in programming \cite{democr1, democr2}, open-source code available online or produced by large language models, often fails to meet software security standards, potentially containing vulnerabilities in around 40\% of cases. \cite{pearce2022asleep}.
More concerning is the training data of generative AI models, deeply rooted in the same insecure public repositories. 
%As a result, unless trained explicitly with security in mind, generative AI models (for automated code generation) gives rise to a vicious cycle of generating and disseminating more insecure code. Since the use of external code persists from novice to experienced developers, the possibility of spreading vulnerable code across various applications remains high.



Security issues can permeate within a application during different phases of its software development lifecycle. The ideal development lifecycle of a software application includes design, implementation, developer testing, code analysis, and code review phases \cite{assal2018security}. While the developer testing and code analysis phase contribute to functional testing of the code, security or vulnerability testing of code occurs primarily during the code review phase. \mj{I am not sure what is the point of the lines appearing before?} While security is sometimes seen as a burden in startup companies, in larger companies, it is considered a necessary evil to protect the company's products. Larger companies properly manage software development lifecycle, but small businesses or startups need to adequately implement better cyber security practices; otherwise, it leaves them susceptible to cyber-attacks \cite{chidukwani2022survey}. It is reported that about 60\% of small businesses that were victims of cyberattacks went out of business within six months \cite{galvin2021percent}. This report further demonstrates that small businesses have much to lose if cyber threats materialize, and it is in their best interest to have cyber defenses in place. Research highlights that 28\% of non-compliant victims will likely suffer another breach within two years after the initial attack \cite{vikingcloud} \mj{How is the last sentence related to everything before that? Appears out of place}.


% Issue with developers
While the democratization of code helps with faster progress, the cost of cybersecurity slows down their productivity in the long run.
Code security knowledge among developers plays a crucial role in ensuring the resilience of programs against various attacks. However, it is crucial to acknowledge developers' challenges as they are often seen as "the weakest link in the chain" regarding security \cite{green2016developers}. Developers are responsible for making final decisions on which code goes into production. Recent research highlights the need for comprehensive security support and training for software developers to effectively address these issues \cite{green2016developers, acar2016you}. One study by Assal et al. \cite{assal2019think} specifically examined the human factor in source code security. The survey highlighted the inadequate interaction between software developers and security practices. Similarly, Hermann et al. \cite{weir2020needs} conducted another survey revealing that less than a quarter of 335 successful mobile application developers had access to security experts. Therefore, addressing these issues is crucial to enhancing software development's overall security posture.




At the same time, recent user-focused research suggests that software developers need critical support when addressing security challenges \cite{acar2016you, green2016developers}. While current vulnerability classification and localization play a critical role in discerning the specific location of code failure, they cannot determine the root cause of the vulnerability. \mj{A sentence here describing what we intuitively mean by ``root cause" would help!} This problem is further exacerbated within large-scale applications, potentially comprising millions of lines of code, where crash reproduction can be exceptionally challenging due to environmental discrepancies \cite{bellare1997forward, capobianco2019employing, han2020unicorn} of the system. Although capturing program stack traces or logs \cite{ji2017rain, kang2011dta} might provide insights such as vulnerability-causing inputs or code break locations, the derived results are often incomplete as they do not necessarily identify the root cause of the vulnerability. Consequently, these run-time analyses from stack traces are incredibly lengthy. So they need time to sort them out, diminishing the usability of this method since it requires too much back and forth between code writing and full deployment.



%Our proposed system is the first to integrate an IoT operating systems repository scanner for function extraction using Joern \cite{joern} and a large language model VulCodeT5 to generate descriptions for the developers in repairing vulnerabilities. 
Therefore, in order to clearly understand what the previous systems are missing and what a developer needs, we initially do an extensive survey analysis. The analysis shows the drawbacks of current systems and reveals that a developer needs to understand the root cause of the vulnerability with a proper description of its CWE category. Thus, to find the root cause of the vulnerability, we introduce T5-GCN, a large language model combined with a Graph Convolutional Network (GCN), to find the root cause of the vulnerability along with its classification and localization. Our innovative approach incorporates an explainability-based method to extract the relationship between a vulnerable statement and the statement most contributing to the vulnerability's root cause. Afterward, we conduct a human evaluation to test the usability of our root cause analysis to repair vulnerabilities and how it intuitively increases the developer's knowledge in writing more secure code in the future. Furthermore, we test our system's generalizability by identifying the root cause of N-day and zero-day vulnerabilities. 

%\mj{Talk a bit more about the user study and the study's novelty. That is one of the most important aspect of the paper!}



%To address these challenges, we are the first to introduce VulCodeT5, a large language model for vulnerability localization and causative insights into the vulnerability. Our proposed VulCodeT5 provides GCN \cite{kipf2016semi} architecture powered by a CodeT5 embedding \cite{wang2021codet5} for vulnerability classification and localization, which harnesses the sequential/syntactical structure of tokens and the graphical structure of a programming language, respectively. Furthermore, we incorporate an explainability-based method to extract the relationship between a vulnerable statement and the statement most contributing to the vulnerability's root cause. The efficacy of our system is substantiated through an exhaustive case study \mj{why do you call it a ``case study"? are you evaluating just one use-case here?} analysis, focusing on evaluating 1) the model's classification performance and vulnerable line detection, 2) the effect of the outcome on the developers in writing secure code, and 3) demonstrating the application of our system by identifying the root cause analysis of vulnerability and its ability to identify and localize N-day and zero-day vulnerabilities in the wild. \mj{Talk a bit more about the user-study and the novelty of the study. That is one of the most important aspect of the paper!}


The contributions delineated in this paper are as follows:
\begin{itemize}

    \item We propose an introductory survey analysis to determine the flaws of the current systems and the drawbacks to the developers' security knowledge. Our primary analysis concludes that the root cause of the vulnerability is needed to help developers solve the vulnerability.

    \item In order to find the root cause of vulnerability, we proposed a T5-GCN(Temp. name) that can find the root cause of a vulnerability along with its classification and localization of the existing vulnerability. Furthermore, we do another extensive human evaluation to determine the effectiveness of our system compared to previous ones.

    \item We provide numerical analysis to show the quantitative results of our system. Furthermore, we also test the generalizability of our system in N-day and 0-day applications to identify the root cause of vulnerability in a program.
    
    %\item We introduce a system that performs function-level granularity analysis in source code to classify and localize vulnerabilities using a CodeT5-powered GCN architecture. This includes a novel token-based approach for finding vulnerable blocks of code.
    
    %\item We incorporate an explainability (used different terminology-- root cause/attribution/causal insight-- remove from the introduction) method within our system to identify the root cause of a vulnerability by elucidating the relationship between two statements: one engendering the vulnerability and the other instigating the code break.
    
    %\item We demonstrate a comprehensive use case of our system by demonstrating its effect on software developers. We provided an extensive survey analysis to demonstrate the usability of our system on its effect on developers and how it helps to write better and secure code.
    
    %detecting N-day and zero-day vulnerabilities prevalent in widely used IoT operating systems.
    
    
\end{itemize}
%\vspace{-11mm}

%The organization of the remainder of this paper is outlined as follows: In Section II, we dive deep into the motivation of this work. Then we delve into the relevant literature and previous studies in Section III. Section IV outlines our preliminary work on vulnerability exploitation, setting the groundwork for the subsequent sections. Our innovative methodology is thoroughly discussed in Section V. Section VI then provides an in-depth exposition of our experimental design and results, along with a comprehensive discussion of the findings. We further substantiate our findings with an ablation study, detailed in Section VII. We conclude our work, summarizing our contributions and discussing potential future directions in Section VIII.

%\vspace{-11mm}


==> sections/survey_BK.tex <==
%\subsection{User-Focused Study Design (Survey Design Goes Methodology)}
We designed a user-centric survey to evaluate our proposed system's effectiveness in addressing code vulnerability issues and aiding developers in learning secure coding practices without over-relying on AI tools. Step 1 and 3 in Figure \ref{fig:fig_2} demonstrates the survey analysis we explain here.



\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.70]{images/arch.pdf}
    %\vspace{-0.3cm}
    \caption{Our proposed approach is organized into three pivotal steps (1) Evaluating programmer insights on current state-of-the-art security vulnerabilities; (2) Introducing an LLM-powered diagnostic toolkit that assists programmers in vulnerability remediation; and (3) Garnering programmer feedback on the toolkit's effectiveness.}
    \label{fig:fig_2}
    %\vspace{-3mm}
\end{figure*}
%While our proposed system does not provide any code completions, we provided information to the developers to help them fix any possible vulnerability in their code. Our approach equips developers with insights enabling them to address code vulnerabilities, ensuring they maintain complete control over their code and its underlying logic. We tested our proposed system using undergraduate and graduate students from Computer Science with programming experience from an R1 research university. 



\subsection{Participant Recruitment}

We recruited our participants from the Computer Science department, enlisting both undergraduate and graduate students who have either completed or are currently enrolled in at least one programming language course. The recruitment process involved utilizing the students' mailing list, with the support of the department admin, to send invitation emails. Furthermore, since many of these participants will join the industry after graduation, their selection is strategic, considering they likely possess limited knowledge and training in code security. This demographic allows us to estimate the effect of insufficient code security knowledge among emerging professionals.

We selected participants with a wide range of educational backgrounds: 1) Undergraduate Students with programming experience, 2) Graduate Students without industry experience, 3) Graduate Students with industry experience, and 4) Graduate Students with research experience. The recruitment process emphasized evaluating their code-writing quality, and therefore, we deliberately omitted the focus on code security practices in our survey. This omission aimed to prevent potential bias, as participants could have otherwise prepared in advance, skewing the results. 
Each participant received a compensation of US\$25 for their contribution to the study. This study involved human participants and was approved by the institution’s Institutional Review Board (IRB).




%The study commenced with participants tackling programming tasks, each embedded with potential Common Weakness Enumeration (CWE) vulnerabilities. These tasks were designed in the C/C++ programming language to ensure consistency (what consistency?) in evaluation. Furthermore, we chose C/C++ as the programming language for our survey since many memory and resource-related vulnerabilities directly arise from it \cite{msrc}.

For a broader understanding of the impact of our proposed system, participants were randomly allocated to two distinct groups: the Control Group and the Assisted Group. Participants were furnished with four types of information based on which category they fall into 1) the specific vulnerable line(s) of code, 2) the vulnerability category, 3) the description of the category, and 4) the root cause of the vulnerability. The control group was provided with the vulnerable line and its associated category. In contrast, the assisted group was provided with the root cause of the vulnerability and the description, along with classification and localization.

%The control group imitates the current state-of-the-art methods, including assisting the developers by providing localization as the highest level of information. However, the assisted group imitates our proposed system, where the developers are provided with the root cause of the vulnerability and a description that helps them understand the vulnerability in the code. We hypothesize that a clear comprehension of the vulnerabilities, supported by their classifications and detailed descriptions, will empower developers to amend the code adeptly, obviating the need for additional resources.






\subsection{Survey Design}

Our survey is structured in two stages to rigorously evaluate our model's effectiveness and usability: The baseline and the evaluation stages.


%\textbf{Learning Stage:} 
%Randomly assigned to the controlled or assisted groups, participants tackled 10 code vulnerability problems. The controlled group received vulnerability localization and classification, while the assisted group additionally gained insights into the root causes. We assume this division will cause some participants to learn and generalize code vulnerability better. After showing them the training codes, we provide the users with some exercise problems to understand how efficiently they are fixing vulnerabilities.




\paragraph{\textbf{Baseline Stage}} In the baseline stage, we asked participants from assisted and control groups to complete ten C functions associated with a grocery store management system. The participants must download a C source file containing skeletal code (i.e., a function declaration without implementation)for each function, accompanied by implementation instructions, parameter and return value details, and example usages. Participants were required to document the start and completion times for each function. Listing \ref{lst:listing-cpp} illustrates one of the ten functions awaiting participant implementation. The tasks involved core C programming concepts like file I/O and memory management. However, we ensured that the implementations of these functions steer clear of advanced data structures to avoid unnecessary complicacy. Essential C libraries and user-defined structures were provided with the skeleton code beforehand. Participants were neither encouraged nor discouraged about using and utilizing resources from online or any code-generative AI, and they could use any code editor or IDE based on their personal preferences. The baseline stage was done in Subsection \ref{moti_1}

%Participants could consult online resources and utilize any text editor or IDE based on their preferences. 


\lstinputlisting[style=CStyle, label={lst:listing-cpp}, caption=Problem 1: A function that primarily checks if the participant handled integer overflow and properly set up a base case to avoid a stack overflow if solved recursively.]{code/problem1.c}


Furthermore, we provided the control group five functions intentionally associated with a particular CWE number. This means, that if the participant makes any security mistake, it would be tied to that CWE number. We provided the two outcomes provided by the SOTA techniques. They were the vulnerable line and the CWE category of the vulnerability. The task was to resolve vulnerability with the given information. We conducted this part of the survey in Subsection \ref{moti_2}.


\paragraph{\textbf{Evaluation Stage}}
In this stage, we assess the participants' ability to repair code and extend the knowledge they have acquired regarding the rectification of security-related code vulnerabilities. The assessment revolves around the five functions we previously provided to the control group. However, this time, the outcomes we provided to the assisted group were the localized vulnerable line, CWE class with description, and the root cause of vulnerability. We asked the assisted group to repair the given five codes. Furthermore, we asked the developers from both groups to rewrite the ten functions they previously wrote to fix any possible security issues they wrote in the baseline stage. The goal was to determine how developers from both groups improved their knowledge using SOTA methods in the control group compared to our technique in the assisted group. This part was done in Subsection \ref{rq1}.

%\color{red}
%(WIP)We described the flow of our survey in Appendix \ref{9_appendix}.
%\color{black}



\subsection{Survey Workflow}

We initially directed participants to complete ten functions within an incomplete C source code file. Notably, the participants needed to be more apprised of the deliberate design of these functions. These functions were intentionally crafted in a manner where potential vulnerabilities could be introduced if not approached with caution. Eligibility criteria for participation necessitated a fundamental understanding of the C programming language, ensuring that the tasks were within the participants' grasp. It is important to emphasize that the ten functions exclusively revolved around elementary C programming concepts and excluded intricate topics like data structures. In cases where participants did not fulfill any of the functions, they were gracefully guided to the survey's conclusion. This approach aimed to maintain a consistent and relevant experience for all participants. Listing \ref{lst:lst2} shows the header file and the structure we provided to the participants.

Furthermore, \ref{lst:lst3} and \ref{lst:lst4} exemplify some other code samples provided to the participants. These are empty functions with a proper description of the problem, a sample test case of the solution, and a clarification on the return type. Furthermore, inside the function body, there is an option to put the starting and ending times to measure how long it took them to complete the function.


If participants made partial progress on the coding assignment, a series of inquiries ensued regarding their familiarity with code vulnerabilities and the extent of their formal cybersecurity training. Following the collection of security-related background information, participants were assigned to either "Form A" or "Form B," with "Form A" representing the assisted group and "Form B" serving as the control group. The survey structure was thoughtfully arranged such that every alternate participant received "Form B," a measure intended to achieve an equitable distribution of approximately 50\% between the control and assisted groups.



Irrespective of the assigned form, participants were presented with five distinct C functions, which they were asked to repair. The control group only had visibility to the CWE class of the vulnerability and the vulnerable line, as depicted in Figure \ref{fig:survey_sota}. However, the assisted group was provided with the CWE category of the vulnerability with a static description, the vulnerable line, and the root cause of the vulnerability as depicted in Figure \ref{fig:survey_our}.



Upon completing the vulnerability assessment task, participants were further probed with questions assessing their confidence levels in mitigating code vulnerabilities and whether they sought assistance from ChatGPT for code composition. The survey concluded with the collection of pertinent demographic data from each participant.



%previously posed in Section \ref{1.5_motivation}. At this juncture, each participant is evaluated under the same criteria, irrespective of their initial grouping (controlled or assisted).

%This stage is designed to gauge the participants’ capability to independently analyze and rectify code vulnerabilities without the assistance of AI tools information like classification, localization, or root cause.







%Given the focus of our survey on the security implications of unsafe code, we selected C as the study language. This choice stems from the ease of inadvertently introducing memory-related bugs in C, such as buffer overflows and null pointer dereferences. Languages like Java or Python handle such bugs differently, offering built-in safeguards and detection mechanisms. A basic understanding of C was a prerequisite for all participants.








%The initial function evaluates the possible combinations of purchasable items, designed to identify unintended stack or integer overflows and assess input validation. Functions 2-5 entail reading and writing to a newline-delimited file, which serves as the grocery store's database system. These tasks are susceptible to a range of vulnerabilities; however, they are designed to assess whether participants can adeptly open and close system resources, effectively load and retrieve contents from the file using a buffer, and allocate dynamic memory appropriately. The remaining functions (6-10) focus on user management within the store system, evaluating skills in string handling, array allocation/deallocation, and buffer length and capacity verification. Participants are not provided assumptions or warned of potential edge cases to check for in any functions.









\subsection{Code Assessment}
We employed a dual-method evaluation approach to assess the participants' code regarding security and functionality. Furthermore, we categorized identified bugs according to their CWE classification \cite{cwe}.

\paragraph{\textbf{Run-time Analysis}} For the run-time of the code written by the participants, we generated two sets of test cases for each function—the first set aimed at evaluating the functionality, ensuring that the code meets the intended requirements. The second, more intricate set was designed to unveil potential vulnerabilities, with specific inputs crafted to induce run-time errors if vulnerabilities were present. A function passing all test cases, functionality, and security was deemed free of vulnerabilities.



\paragraph{\textbf{Manual Analysis}} While most participants submitted a fully working code, some provided partially written non-compilable code. Furthermore, some participants also use pseudocode as a solution to vulnerability. Therefore, we also do a manual code review by our internal security experts to identify potential vulnerabilities and fixes. Our security experts initially manually check the functionality by reading code and try to estimate the outcome based on some input test cases. Furthermore, for security testing, our security experts check whether the function would fall into a runtime error in the case of NULL, negative, or overloading numerical limits in the code. Based on the partially written code or pseudocode, if the function is possibly breaking at these inputs, the security experts deem it as a vulnerable function.






==> sections/threat_model.tex <==


%\textbf{Threat Model:}
In exploring our threat model, we primarily consider two types of actors in the software development landscape. The first category comprises malicious actors posing as legitimate developers who post vulnerable source code or snippets on developer collaboration platforms, such as GitHub or StackOverflow \cite{log4j}. The second group includes authentic developers who, unaware of the security implications, incorporate this vulnerable code from online platforms into their IoT software development projects.


Our threat model primarily focuses on vulnerabilities at the operating system or application level, with an assumption of reliable and trustworthy hardware and kernel for IoT devices. The vulnerabilities at these levels could compromise the physical memory and CPU caches by gaining privileged root mode access. The attackers could exploit such vulnerabilities through various attack scenarios, like buffer overflow, code injection, or improper operations within a memory buffer. These vulnerabilities can subsequently provide control over the system, enable data theft, or even launch further attacks. Our approach to minimizing vulnerability is twofold. We propose an LLM-based generative model with a description to aid developers in solving vulnerabilities. Moreover, we complement vulnerability description with classification and localization of the root cause of the vulnerability to help the developers fix them. 

\begin{comment}
% \usepackage{booktabs}
\begin{table}[H]
\centering
\caption{A survey on how the outcome of different SOTA models helps security experts and developers in determining the vulnerability}
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{SOTA Model} & \textbf{Task/Output}    & \textbf{Security Experts} & \textbf{Developers} & \textbf{Suggestion} \\ \midrule
Devign     & Detection      & 34\%             & 28\%      & Localization \\
PFGCN      & Classification & 57\%             & 37\%      & Description of CWE \\
VELVET     & Localization   & 71\%             & 60\%      & Description on how to fix \\ \bottomrule
\end{tabular}
\label{tab:survey_1}
\end{table}
\end{comment}



